G-SemTMO: Tone Mapping with a Trainable Semantic Graph

A Tone Mapping Operator (TMO) is required to render images with a High Dynamic Range (HDR) on media with limited dynamic capabilities. TMOs compress the dynamic range with the aim of preserving the visually perceptual cues of the scene. Previous literature has established the benefits of TMOs being semantic aware, understanding the content in the scene to preserve the cues better. Expert photographers analyze the semantic and the contextual information of a scene and decide tonal transformations or local luminance adjustments. This process can be considered a manual analogy to tone mapping. In this work, we draw inspiration from an expert photographer's approach and present a Graph-based Semantic-aware Tone Mapping Operator, G-SemTMO. We leverage semantic information as well as the contextual information of the scene in the form of a graph capturing the spatial arrangements of its semantic segments. Using Graph Convolutional Network (GCN), we predict intermediate parameters called Semantic Hints and use these parameters to apply tonal adjustments locally to different semantic segments in the image. In addition, we also introduce LocHDR, a dataset of 781 HDR images tone mapped manually by an expert photo-retoucher with local tonal enhancements. We conduct ablation studies to show that our approach, G-SemTMO\footnote{Code and dataset to be published with the final version of the manuscript}, can learn both global and local tonal transformations from a pair of input linear and manually retouched images by leveraging the semantic graphs and produce better results than both classical and learning based TMOs. We also conduct ablation experiments to validate the advantage of using GCN.

==> Biblio.tex <==
@article{wu2019fastfcn,
  title={{FastFCN: Rethinking dilated convolution in the backbone for semantic segmentation}},
  author={Huikai Wu and Junge Zhang and Kaiqi Huang and Kongming Liang and Yizhou Yu},
  journal={arXiv preprint arXiv:1903.11816},
  year={2019}
}

@inproceedings{fivek,
  title={Learning photographic global tonal adjustment with a database of input/output image pairs},
  author={Bychkovsky, Vladimir and Paris, Sylvain and Chan, Eric and Durand, Fr{\'e}do},
  booktitle={CVPR 2011},
  pages={97--104},
  year={2011},
  organization={IEEE}
}
@article{ade20k,
  title={{Semantic Understanding of Scenes through the ADE20K Dataset}},
  author={Bolei Zhou and Hang Zhao and Xavier Puig and Tete Xiao and Sanja Fidler and Adela Barriuso and Antonio Torralba},
  journal={International Journal of Computer Vision},
  volume={127},
  number={3},
  pages={302--321},
  year={2019},
  publisher={Springer}
}

@inproceedings{goswami2020tone,
  title={{Tone Mapping Operators: Progressing Towards Semantic-awareness}},
  author={Abhishek Goswami and Mathis Petrovich and Wolf Hauser and Fr{\'e}d{\'e}ric Dufaux},
  booktitle={2020 IEEE International Conference on Multimedia \& Expo Workshops (ICMEW)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}
@article{yan2016automatic,
  title={{Automatic Photo Adjustment using Deep Neural Networks}},
  author={Zhicheng Yan and Hao Zhang and Baoyuan Wang and Sylvain Paris and Yizhou Yu},
  journal={ACM Transactions on Graphics (TOG)},
  volume={35},
  number={2},
  pages={1--15},
  year={2016},
  publisher={ACM New York, NY, USA}
}
@inproceedings{hwang2012context,
  title={{Context-based Automatic Local Image Enhancement}},
  author={Sung Ju Hwang and Ashish Kapoor and Sing Bing Kang},
  booktitle={European conference on computer vision},
  pages={569--582},
  year={2012},
  organization={Springer}
}
@article{gharbi2017deep,
  title={{Deep Bilateral Learning for Real-Time Image Enhancement}},
  author={Micha{\"e}l Gharbi and Jiawen Chen and Jonathan T Barron and Samuel W Hasinoff and Fr{\'e}do Durand},
  journal={ACM Transactions on Graphics (TOG)},
  volume={36},
  number={4},
  pages={118},
  year={2017},
  publisher={ACM}
}

@article{rong2019dropedge,
  title={{Dropedge: Towards deep graph convolutional networks on node classification}},
  author={Yu Rong and Wenbing Huang and Tingyang Xu and Junzhou Huang},
  journal={arXiv preprint arXiv:1907.10903},
  year={2019}
}

@article{GastalOliveira2010SharedMatting,
  author  = {Eduardo S. L. Gastal and Manuel M. Oliveira},
  title   = {{Shared Sampling for Real-Time Alpha Matting}},
  journal = {Computer Graphics Forum},
  volume  = {29},
  number  = {2},
  month   = {May},
  year    = {2010},
  pages   = {575-584},
  note    = {Proceedings of Eurographics}
}

@misc{adamw,
      title={{Decoupled Weight Decay Regularization}}, 
      author={Ilya Loshchilov and Frank Hutter},
      year={2019},
      eprint={1711.05101},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}
  
@incollection{NEURIPS2019_9015,
title = {{PyTorch: An Imperative Style, High-Performance Deep Learning Library}},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
}

@inproceedings{Fey/Lenssen/2019,
  title={{Fast Graph Representation Learning with PyTorch Geometric}},
  author={Fey, Matthias and Lenssen, Jan E.},
  booktitle={ICLR Workshop on Representation Learning on Graphs and Manifolds},
  year={2019},
}
@misc{kipf2017semisupervised,
      title={{Semi-Supervised Classification with Graph Convolutional Networks}}, 
      author={Thomas N. Kipf and Max Welling},
      year={2017},
      eprint={1609.02907},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@incollection{mantiuk2008display,
  title={{Display Adaptive Tone Mapping}},
  author={Mantiuk, Rafa{\l} and Daly, Scott and Kerofsky, Louis},
  booktitle={ACM SIGGRAPH 2008 papers},
  pages={1--10},
  year={2008}
}
@inproceedings{durand2002fast,
  title={{Fast Bilateral Filtering for the Display of High-Dynamic-Range Images}},
  author={Durand, Fredo and Dorsey, Julie},
  booktitle={ACM transactions on graphics (TOG)},
  volume={21},
  number={3},
  pages={257--266},
  year={2002},
  organization={ACM}
}
@inproceedings{reinhard2002photographic,
  title={{Photographic Tone Reproduction for Digital Images}},
  author={Reinhard, Erik and Stark, Michael and Shirley, Peter and Ferwerda, James},
  booktitle={Proceedings of the 29th annual conference on Computer graphics and interactive techniques},
  pages={267--276},
  year={2002}
}
@article{reinhard2005dynamic,
  title={{Dynamic Range Reduction Inspired by Photoreceptor Physiology}},
  author={Reinhard, Erik and Devlin, Kate},
  journal={IEEE transactions on visualization and computer graphics},
  volume={11},
  number={1},
  pages={13--24},
  year={2005},
  publisher={IEEE}
}
@article{Kaufman-CAPE-2012,
    author  = {Liad Kaufman and Dani Lischinski and Michael Werman},
    title   = {{Content-Aware Automatic Photo Enhancement}},
    year    = {2012},
    journal = {Computer Graphics Forum},
    volume  = {31},
    number  = {8},
    pages   = {2528--2540}
}

@INPROCEEDINGS{Krawczyk05EG,
AUTHOR = {Krawczyk, Grzegorz and Myszkowski, Karol and Seidel, Hans-Peter},
TITLE = {{Lightness Perception in Tone Reproduction for High Dynamic Range Images}},
BOOKTITLE = {The European Association for Computer Graphics 26th Annual Conference EUROGRAPHICS 2005},
PUBLISHER = {Blackwell},
YEAR = {2005},
NUMBER = {3},
VOLUME = {24},
PAGES = {xx--xx},
SERIES = {Computer Graphics Forum},
ADDRESS = {Dublin, Ireland},
}
@article{zhou2020graph,
  title={{Graph neural networks: A Review of Methods and Applications}},
  author={Zhou, Jie and Cui, Ganqu and Hu, Shengding and Zhang, Zhengyan and Yang, Cheng and Liu, Zhiyuan and Wang, Lifeng and Li, Changcheng and Sun, Maosong},
  journal={AI Open},
  volume={1},
  pages={57--81},
  year={2020},
  publisher={Elsevier}
}

@misc{pfstools,
  author = {Rafal Mantiuk and Grzegorz Krawczyk},
  title = {PfsTmo},
  url = {http://pfstools.sourceforge.net/pfstmo.html},
  note = {Accessed: 2021-05-07}
}
@article{abasi2020distance,
  title={Distance metrics for very large color differences},
  author={Abasi, Saeedeh and Amani Tehran, Mohammad and Fairchild, Mark D},
  journal={Color Research \& Application},
  volume={45},
  number={2},
  pages={208--223},
  year={2020},
  publisher={Wiley Online Library}
}
@inproceedings{wang2003multiscale,
  title={{Multiscale Structural Similarity for Image Quality Assessment}},
  author={Wang, Zhou and Simoncelli, Eero P and Bovik, Alan C},
  booktitle={The Thirty-Seventh Asilomar Conference on Signals, Systems \& Computers, 2003},
  volume={2},
  pages={1398--1402},
  year={2003},
  organization={Ieee}
}
@article{mantiuk2011hdr,
  title={{HDR-VDP-2: A calibrated visual metric for visibility and quality predictions in all luminance conditions}},
  author={Mantiuk, Rafa{\l} and Kim, Kil Joong and Rempel, Allan G and Heidrich, Wolfgang},
  journal={ACM Transactions on graphics (TOG)},
  volume={30},
  number={4},
  pages={1--14},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@INPROCEEDINGS{wang_classification,
  author={Wang, Xiaolong and Ye, Yufei and Gupta, Abhinav},
  booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 
  title={{Zero-Shot Recognition via Semantic Embeddings and Knowledge Graphs}}, 
  year={2018},
  volume={},
  number={},
  pages={6857-6866},
  doi={10.1109/CVPR.2018.00717}}
  
@inproceedings{kampffmeyer2019rethinking,
  title={{Rethinking Knowledge Graph Propagation for Zero-Shot Learning}},
  author={Kampffmeyer, Michael and Chen, Yinbo and Liang, Xiaodan and Wang, Hao and Zhang, Yujia and Xing, Eric P},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11487--11496},
  year={2019}
}
@article{wang2018deep,
  title={{Deep Reasoning with Knowledge Graph for Social Relationship Understanding}},
  author={Wang, Zhouxia and Chen, Tianshui and Ren, Jimmy and Yu, Weihao and Cheng, Hui and Lin, Liang},
  journal={arXiv preprint arXiv:1807.00504},
  year={2018}
}
@inproceedings{liang2016semantic,
  title={{Semantic Object Parsing with Graph LSTM}},
  author={Liang, Xiaodan and Shen, Xiaohui and Feng, Jiashi and Lin, Liang and Yan, Shuicheng},
  booktitle={European Conference on Computer Vision},
  pages={125--143},
  year={2016},
  organization={Springer}
}
@inproceedings{Fairchild,
  title={{The HDR photographic survey}},
  author={Fairchild, Mark D},
  booktitle={Color and imaging conference},
  volume={2007},
  number={1},
  pages={233--238},
  year={2007},
  organization={Society for Imaging Science and Technology}
}

@inproceedings{Montulet2019,
author = {Montulet, Rico and Briassouli, Alexia and Maastricht, N.},
booktitle = {BMVC},
file = {:C\:/Users/manti/Dropbox/mendeley_papers/Montulet, Briassouli, Maastricht/BMVC/Montulet, Briassouli, Maastricht - 2019 - Deep Learning for Robust end-to-end Tone Mapping.pdf:pdf},
mendeley-groups = {Tone mapping/Learning based},
pages = {194},
title = {{Deep Learning for Robust end-to-end Tone Mapping}},
year = {2019}
}

@article{Rana2020,
author = {Rana, Aakanksha and Singh, Praveer and Valenzise, Giuseppe and Dufaux, Frederic and Komodakis, Nikos and Smolic, Aljosa},
doi = {10.1109/TIP.2019.2936649},
issn = {1057-7149},
journal = {IEEE Transactions on Image Processing},
mendeley-groups = {Tone mapping/Learning based},
pages = {1285--1298},
title = {{Deep Tone Mapping Operator for High Dynamic Range Images}},
url = {https://ieeexplore.ieee.org/document/8822603/},
volume = {29},
year = {2020}
}

@article{Yeganeh2013a,
author = {Yeganeh, Hojatollah and Wang, Zhou},
doi = {10.1109/TIP.2012.2221725},
issn = {1057-7149},
journal = {IEEE Transactions on Image Processing},
keywords = {TMQI},
mendeley-groups = {Tone mapping/Tone-mapping metrics},
mendeley-tags = {TMQI},
month = {feb},
number = {2},
pages = {657--667},
title = {{Objective Quality Assessment of Tone-Mapped Images}},
url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=6319406},
volume = {22},
year = {2013}
}

@article{Hullin2011,
author = {Hullin, Matthias and Eisemann, Elmar and Seidel, Hans-Peter and Lee, Sungkil},
doi = {10.1145/2010324.1965003},
issn = {07300301},
journal = {ACM Transactions on Graphics},
mendeley-groups = {Tone mapping/Camera simulation},
month = {jul},
number = {4},
pages = {1},
title = {{Physically-based Real-Time Lens Flare Rendering}},
url = {http://portal.acm.org/citation.cfm?doid=2010324.1965003},
volume = {30},
year = {2011}
}

@article{Wanat2014,
author = {Wanat, Robert and Mantiuk, Rafal K},
doi = {10.1145/2601097.2601150},
journal = {ACM Transactions on Graphics (Proc. of SIGGRAPH)},
keywords = {backlight dimming,color perception,computational display,contrast perception,low,luminance display,retargeting},
number = {4},
pages = {147},
title = {{Simulating and compensating changes in appearance between day and night vision}},
volume = {33},
year = {2014}
}

@article{Irawan2005,
author = {Irawan, P and Ferwerda, JA and Marschner, SR},
doi = {10.2312/EGWR/EGSR05/231-242},
journal = {EGSR},
keywords = {temporal},
mendeley-groups = {Tone mapping,Light adaptation},
mendeley-tags = {temporal},
title = {{Perceptually Based Tone Mapping of High Dynamic Range Image Streams}},
year = {2005}
}

@misc{SMPTE2017,
author = {SMPTE},
doi = {10.5594/SMPTE.ST2094-2.2017},
title = {{ST 2094-2:2017 Dynamic Metadata for Color Volume Transform — KLV Encoding and MXF Mapping}},
year = {2017}
}


@article{KedeMa2015,
author = {{Kede Ma} and Yeganeh, Hojatollah and {Kai Zeng} and {Zhou Wang}},
doi = {10.1109/TIP.2015.2436340},
issn = {1057-7149},
journal = {IEEE Transactions on Image Processing},
mendeley-groups = {Tone mapping/Optimization based},
month = {oct},
number = {10},
pages = {3086--3097},
title = {{High Dynamic Range Image Compression by Optimizing Tone Mapped Image Quality Index}},
url = {http://ieeexplore.ieee.org/document/7111279/},
volume = {24},
year = {2015}
}

@ARTICLE{mle,
  author={Zhang, Wei and Martin, Ralph R. and Liu, Hantao},
  journal={IEEE Transactions on Circuits and Systems for Video Technology}, 
  title={{A Saliency Dispersion Measure for Improving Saliency-Based Image Quality Metrics}}, 
  year={2018},
  volume={28},
  number={6},
  pages={1462-1466},
  doi={10.1109/TCSVT.2017.2650910}} 
  
@book{friedman2001elements,
  title={{The Elements of Statistical Learning}},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  volume={1},
  number={10},
  year={2001},
  publisher={Springer series in statistics New York}
}

@book{ansel1983print,
  title={{The Print. Vol. 3. The Ansel Adams photography series}},
  author={Adams, Ansel},
  year={1983},
  publisher={Boston: Little, Brown and Company.}
}

@misc{jinchen,
  author = {Jinchen Ge},
  title = {{HDRnet-PyTorch}},
  url = {https://github.com/gejinchen/HDRnet-PyTorch},
  note = {Accessed: 2022-07-13}
}
